Multipath-based SLAM with Cooperation and Map Fusion in MIMO Systems

Multipath-based simultaneous localization and mapping (MP-SLAM) is a promising approach in wireless networks for obtaining position information of transmitters and receivers as well as information on the propagation environment. MP-SLAM models specular reflections of radio frequency (RF) signals at flat surfaces as virtual anchors (VAs), the mirror images of base stations (BSs). Conventional methods for MP-SLAM consider a single mobile terminal (MT) which has to be localized. The availability of additional MTs paves the way for utilizing additional information in the scenario. Specifically enabling MTs to exchange information allows for data fusion over different observations of VAs made by different MTs. Furthermore, cooperative localization becomes possible in addition to multipathbased localization. Utilizing this additional information enables more robust mapping and higher localization accuracy.

==> biography.tex <==
%\newpage
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/wielandner.jpeg}}]{Lukas~Wielandner} (S'20) received his Dipl.-Ing. (MSc.) degree in technical physics from Graz University of Technology, Austria, in 2018.  
He received his Ph.D. degree in electrical engineering at the Signal Processing and Speech Communication Laboratory (SPSC) of Graz University of Technology, Austria  in 2022. His research interests include localization and navigation, estimation/detection theory, inference on graphs and iterative message passing algorithms. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=25mm,height=32.15mm,clip,keepaspectratio]{bio_pics/alexander_venus_small.jpg}}]{Alexander~Venus} (S'20) received his B.Sc. and  Dipl.-Ing.\ (M.Sc.\ ) degrees (with highest honors) in biomedical engineering and information and communication engineering from Graz University of Technology, Austria in 2012 and 2015, respectively. He was a research and development engineer at Anton Paar GmbH, Graz from 2014 to 2019. He is currently a project assistant at Graz University of Technology, where he is pursuing his Ph.D. degree.
	
His research interests include radio-based localization and navigation, statistical signal processing, estimation/detection theory, machine learning and error bounds. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/ThomasWilding.jpeg}}]{Thomas Wilding}
(S'17) received his B.Sc. and  Dipl.-Ing.\ (M.Sc.) degrees in audio and electrical engineering from the University of Music and Performing Arts Graz, Austria in 2013 and 2016, respectively, and his Ph.D.\ from Graz University of Technology, Austria in 2022. He is currently a post-doctoral researcher at Graz University of Technology working on positioning, sensing and environment learning in wireless systems.
%
His research interests include radio localization and navigation, graphical models and data fusion. 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/ErikLeitinger_Photo.jpg}}]{Erik~Leitinger} (Member, IEEE)received his MSc and PhD degrees (with highest honors) in electrical engineering from Graz University of Technology, Austria in 2012 and 2016, respectively. He was postdoctoral researcher at the department of Electrical and Information Technology at Lund University from 2016 to 2018. He is currently a University Assistant at Graz University of Technology. Dr. Leitinger served as co-chair of the special session "Synergistic Radar Signal Processing and Tracking" at the IEEE Radar Conference in 2021. He is co-organizer of the special issue "Graph-Based Localization and Tracking" in the Journal of Advances in Information Fusion (JAIF). Dr.\ Leitinger received an Award of Excellence from the Federal Ministry of Science, Research and Economy (BMWFW) for his PhD Thesis. He is an Erwin Schr\"odinger Fellow. His research interests include inference on graphs, localization and navigation, machine learning, multiagent systems, stochastic modeling and estimation of radio channels, and estimation/detection theory. 
\end{IEEEbiography}






==> definitions.tex <==
%!TEX root = ./JAIF_2023_V3.tex

\usepackage{amsthm,amsmath,array}   
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{color}
\usepackage{xcolor}
\usepackage{cite}
\usepackage{bm}
\usepackage{epsfig,psfrag}
\usepackage{tabularx}
\usepackage{acronym}
\usepackage[yyyymmdd,hhmmss]{datetime}
\usepackage{bbm}
\usepackage{notation}
\usepackage{mathrsfs} 
\usepackage{bardiag}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{colortbl,pgfplotstable}
\usepackage{dsfont}
\usepackage{times}
\usepackage{rotating}
\usepackage{enumitem}

\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\SetKwRepeat{Do}{do}{while}

\usepackage[caption=false,font=footnotesize]{subfig}

\usepackage{pgfplots}
\usepackage{tikzscale}
\usepackage{tikz}



% tikz packages
\usetikzlibrary{shapes.misc}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{angles}
\usetikzlibrary{quotes}
\usetikzlibrary{fit}
\usetikzlibrary{graphs}
\usetikzlibrary{patterns}
\usetikzlibrary{petri}
\usetikzlibrary{plotmarks}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{decorations.shapes}
\usetikzlibrary{decorations.text}
\usetikzlibrary{backgrounds}
\usetikzlibrary{calc}
\usetikzlibrary{spy}
\usetikzlibrary{shapes,arrows}

\usepackage{tikzscale}

% pgf packages
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{colormaps}
\usepgfplotslibrary{patchplots}
\usepgfplotslibrary{units}


\usepackage[most,theorems]{tcolorbox}
\tcbuselibrary{most}
\tcbset{every box/.style={enhanced,breakable},shield externalize}


\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{magenta_}{rgb}{1.0, 0, 1.0}
\newcommand{\psfragoffset}[6]{\psfrag{#1}{#2 \textcolor{#3}{\raisebox{#5em}{\hspace{#4em}#6}}}}
\definecolor{darkgrey}{rgb}{0.3, 0.3, 0.3}
\newcommand{\rd}{\textcolor{red}}
\newcommand{\bl}{\textcolor{blue}}
\newcommand{\dgr}{\textcolor{darkgreen}}
\newcommand{\mg}{\textcolor{magenta}}

\newcommand{\eq}{\,=\,}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ist}{\hspace*{.3mm}}
\newcommand{\rmv}{\hspace*{-.3mm}}
\newcommand{\iist}{\hspace*{1mm}}
\newcommand{\rrmv}{\hspace*{-1mm}}
\newcommand{\rreq}{\hspace*{-1mm}= \hspace*{-1mm}}
\newcommand{\bd}[1]{\mathbf{#1}}
\newcommand{\cl}[1]{\mathcal{#1}}
\newcommand{\nn}{\nonumber}

\newcommand{\com}[1]{{\color{blue} [#1]}}%my comments
\newcommand{\discuss}[1]{{\color{purple}  #1 (discuss)}}

\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\interdisplaylinepenalty=2500
\allowdisplaybreaks
\sloppy



\newcommand{\ticked}{$\text{\rlap{$\checkmark$}}\square$}
\newcommand{\unticked}{{$\square$}}
\newcommand{\tick}[1]{\ifthenelse{#1=1}{\ticked}{\unticked}}

\newcommand{\vm}[1]{\ensuremath{\bm{#1}}}


\providecommand{\bl}{\textcolor{blue}}
\providecommand{\rd}{\textcolor{red}}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}
\providecommand{\eq}{\,=\,}
\providecommand{\ist}{\hspace*{.3mm}}
\providecommand{\isti}{\hspace*{.4mm}}
\providecommand{\rmv}{\hspace*{-.3mm}}
\providecommand{\iist}{\hspace*{1mm}}
\providecommand{\rrmv}{\hspace*{-1mm}}
\providecommand{\nn}{\nonumber}
\providecommand{\aa}{\lambda}
\providecommand{\bb}{\nu}
\newcommand{\T}{\text{T}}
\newcommand{\as}{\va{a}}	
\newcommand{\va}[1]{#1} 						
\newcommand{\bs}{\va{b}}

\providecommand{\highlight}[1]{\textcolor{blue}{#1}}
\providecommand{\pbs}[1]{\scriptscriptstyle #1}
\providecommand{\todo}[1]{\textcolor{red}{\textbf{ToDo:  }#1}}

\definecolor{colA}{rgb}{0,0,1}% blue 
\definecolor{colB}{rgb}{0.5,0.0,0.5}% purple
\definecolor{colC}{rgb}{0,0.5,0}% green
\definecolor{colD}{rgb}{0.1333,0.5451,0.1333}% green
\definecolor{colE}{rgb}{1.00000,0.55,0.00000}% dark-orange
\definecolor{colF}{rgb}{1.00000,0.0,0.00000}% red
\definecolor{col_mag}{rgb}{1.00000,0.00000,1.00000}% magenta
\definecolor{col_cyan}{rgb}{0,1,1}% cyan
\definecolor{col_grey}{rgb}{0.4,0.4,0.4}% grey
\definecolor{col_grey2}{rgb}{0.6,0.6,0.6}% grey
\definecolor{lightgray}{rgb}{0.9,0.9,0.9}  
\definecolor{Gray}{rgb}{225, 225, 225} 
\definecolor{matlabBlue}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{matlabOrange}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{matlabYellow}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{matlabLila}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{matlabGreen}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{col_PAgreen}{rgb}{0.00000,0.49800,0.00000}%

\def\linewidthA{0.5}
\def\linewidthB{1}
\def\linewidthC{0.3}
\def\linewidthD{0.7}

\def\mylinewidth{0.7}
\def\mylinewidth2{1}

\def\figureH{3cm}
\def\figureW{6cm}
\def\figureW2{5cm}

\def\figureCLToy{4cm}

\def\figureWsmall{3.0cm}
\def\figureHsmall{2.0cm}

\def\figureDataW{5cm}
\def\figureDataH{4cm}


\def\marksizeA{1.5}
\def\marksizeB{1.0}
\def\marksizeC{0.7}


\newcommand{\scl}{0.7}
\newcommand{\scli}{0.5}
\newcommand{\sclii}{0.8}

%\newcommand{\bl}{\textcolor{blue}}
%\newcommand{\mo}{\textcolor{matlabOrange}}

%\newcommand{\ps}{$p_{\text{s}}$}
\newcommand{\ps}{p_{\text{s}}}
\newcommand{\mufa}{\mu_{\text{fa}}}
%\newcommand{\mum}{\mu_{\text{m}}}
\newcommand{\ffa}{f_{\text{fa}}}
\newcommand{\Kk}{K^{(j)}_{\scalebox{.8}{$\scriptscriptstyle n \rmv - \rmv 1$}}}



%%%%%%%%%%%%%%%%  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfplotsset{styleA/.style={color=colA, line width=\linewidthA, mark=\markA, mark size=\marksizeA, mark repeat=1, mark phase = 0, mark optiodvipsnamesns={solid}}}
\pgfplotsset{styleB/.style={color=colB, line width=\linewidthA, mark=\markB, mark size=\marksizeA, mark repeat=1, mark phase = 0, mark options={solid}}}
\pgfplotsset{styleC/.style={color=colC, line width=\linewidthA, mark=\markC, mark size=\marksizeA, mark repeat=1, mark phase = 0, mark options={solid}}}
\pgfplotsset{styleD/.style={color=col_cyan, line width=\linewidthA, mark=\markD, mark size=\marksizeA, mark repeat=1, mark phase = 0, mark options={solid}}}
\pgfplotsset{styleE/.style={color=colE, line width=\linewidthA, mark=\markE, mark size=\marksizeA, mark repeat=1, mark phase = 0, mark options={solid}}}
\pgfplotsset{styleF/.style={color=colF, line width=\linewidthA, mark=\markF, mark size=\marksizeA, mark repeat=1, mark phase = 0, mark options={solid}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%% Styles %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfplotsset{styleSLAM0p0/.style={mymarkfixednumber={\markA}{mark size=\marksizeA,solid}{12},color=matlabBlue, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabBlue}}}
\pgfplotsset{styleSLAM0p03/.style={mymarkfixednumber={\markB}{mark size=\marksizeA,solid}{6},color=matlabBlue,dashdotted, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabBlue}}}
\pgfplotsset{styleSLAM0p15/.style={mymarkfixednumber={\markC}{mark size=\marksizeA,solid}{10},color=matlabBlue,densely dashed, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabBlue}}}
\pgfplotsset{styleSLAM0p3/.style={mymarkfixednumber={\markD}{mark size=\marksizeA,solid}{8},color=matlabBlue,densely dotted, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabBlue}}}

\pgfplotsset{styleEFSLAM0p0/.style={mymarkfixednumber={\markAa}{mark size=\marksizeA,solid}{10},color=matlabOrange, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabOrange}}}
\pgfplotsset{styleEFSLAM0p03/.style={mymarkfixednumber={\markBb}{mark size=\marksizeA,solid}{13},color=matlabOrange,dashdotted, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabOrange}}}
\pgfplotsset{styleEFSLAM0p15/.style={mymarkfixednumber={\markCc}{mark size=\marksizeA,solid}{7},color=matlabOrange,densely dashed, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabOrange}}}
\pgfplotsset{styleEFSLAM0p3/.style={mymarkfixednumber={\markDd}{mark size=\marksizeA,solid}{8},color=matlabOrange,densely dotted, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabOrange}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%% CDF Styles %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfplotsset{CDFstyleSLAM0p0/.style={mymarkfixednumber={\markA}{mark size=\marksizeA,solid}{3},color=matlabBlue, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabBlue}}}
\pgfplotsset{CDFstyleSLAM0p03/.style={mymarkfixednumber={\markB}{mark size=\marksizeA,solid}{100},color=matlabBlue,dashdotted, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabBlue}}}
\pgfplotsset{CDFstyleSLAM0p15/.style={mymarkfixednumber={\markC}{mark size=\marksizeA,solid}{40},color=matlabBlue,densely dashed, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabBlue}}}
\pgfplotsset{CDFstyleSLAM0p3/.style={mymarkfixednumber={\markD}{mark size=\marksizeA,solid}{40},color=matlabBlue,densely dotted, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabBlue}}}

\pgfplotsset{CDFstyleEFSLAM0p0/.style={mymarkfixednumber={\markAa}{mark size=\marksizeA,solid}{2},color=matlabOrange, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabOrange}}}
\pgfplotsset{CDFstyleEFSLAM0p03/.style={mymarkfixednumber={\markBb}{mark size=\marksizeA,solid}{4},color=matlabOrange,dashdotted, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabOrange}}}
\pgfplotsset{CDFstyleEFSLAM0p15/.style={mymarkfixednumber={\markCc}{mark size=\marksizeA,solid}{7},color=matlabOrange,densely dashed, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabOrange}}}
\pgfplotsset{CDFstyleEFSLAM0p3/.style={mymarkfixednumber={\markDd}{mark size=\marksizeA,solid}{15},color=matlabOrange,densely dotted, line width=\linewidthA, mark repeat=1, mark phase = 0, mark options={solid,matlabOrange}}}



\pgfdeclarelayer{backback1}
\pgfdeclarelayer{back1}
\pgfdeclarelayer{lay1}
\pgfdeclarelayer{backback2}
\pgfdeclarelayer{back2}
\pgfdeclarelayer{lay2}
\pgfsetlayers{backback2,back2,lay2,backback1,back1,lay1,main}

%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{FGgreen}{RGB}{34,139,34}
\definecolor{FGblue}{RGB}{80,120,255}
\definecolor{FGred}{RGB}{255,110,110}

\colorlet{fgColor_node}{colA}
\colorlet{fgColorUp1}{colB}
\colorlet{fgColor_coop}{colB}
\colorlet{fgColorBG}{colC}
\colorlet{fgColor_facAlpha}{colE}
\colorlet{fgColorPost3}{colF}
\colorlet{fgColorComb}{colE}
\colorlet{fgColorBox}{colE}
\def\WhiteFactor{15}
\def\WhiteFactorBG{10}
\def\WhiteFactorBlack{5}

% **************************************************************************************************
% * MATH
% **************************************************************************************************
\newcommand{\mumN}[2]{\ensuremath{\mu_\text{m}\big(\tilde{\V{x}}_{#2} , \overline{\V{x}}^{(j)}_{#1 , n}\big)}}
\newcommand{\mumL}[2]{\ensuremath{\mu_\text{m}\big(\tilde{\V{x}}_{#2} , \underline{\V{x}}^{(j)}_{#1 , n}\big)}}
\newcommand{\mum}[1]{\ensuremath{\mu_\text{m}\big(\tilde{\V{x}}_n , \V{x}^{(j)}_{#1 , n}\big)}}

\newcommand{\x}{\tilde{\V{x}}_n}
\newcommand{\xn}[1]{\tilde{\V{x}}_{#1}}

\newcommand{\al}{\underline{a}^{(j)}_{kl,n}}
\newcommand{\an}[2]{\overline{a}^{(j)}_{#1 #2,n}}

\newcommand{\Lx}{\underline{\V{x}}^{(j)}_{k,n}}
\newcommand{\Lxn}[1]{\underline{\V{x}}^{(j)}_{k,#1}}
\newcommand{\Nx}[1]{\overline{\V{x}}^{(j)}_{#1,n}}

% signals
\newcommand{\ddelt}[1]{\delta\!\left( #1 \right)} %dirac delta delay
\newcommand{\kdelt}[1]{\delta\!\left[ #1 \right]} %kornecker delta delay

% highlighting
\newcommand{\vms}[1]{\ensuremath{\bm{#1}}} %vector or matrix
% \newcommand{\vm}[1]{\ensuremath{{\bf #1}}} %vector or matrix
\newcommand{\nth}[1]{\ensuremath{#1}-th} %n-th something

% functions
\renewcommand{\exp}[1]{\ensuremath{{e}^{#1}}}% exponential
\newcommand{\expt}[1]{\ensuremath{\text{exp}\,\{#1 \}}}% exponential
\renewcommand{\ln}[1]{\ensuremath{\text{ln}\!\left(#1\right)}}% natural logarithm
%\newcommand{\lnl}[1]{\ensuremath{\text{ln}\,#1}}% natural logarithm for single aruments without brakets
\newcommand{\ld}[1]{\ensuremath{\text{ld}\!\left(#1\right)}}% logarithm base 2
\renewcommand{\log}[1]{\ensuremath{\text{log}\!\left(#1\right)}}% logarithm (base 10)
\newcommand{\logl}[1]{\ensuremath{\text{log}\, #1 }}% logarithm (base 10) without brackets
\newcommand{\logb}[2]{\ensuremath{\text{log}_{#1}\!\left(#2\right)}}% logarithm base ...
\newcommand{\deter}[1]{\ensuremath{\lvert #1 \rvert}} %simple determinant operator

% rounding
\newcommand{\round}[1]{\ensuremath{\text{round}\!\left(#1\right)}}% rounding towards next integer
\newcommand{\ceil}[1]{\ensuremath{\left\lceil#1\right\rceil}}% rounding towards infinity
\newcommand{\floor}[1]{\ensuremath{\left\lfloor#1\right\rfloor}}% rounding towards zero

% operators
%\newcommand{\E}[1]{\ensuremath{\mathbb{E}\!\left[#1\right]}}% expectation operator
\newcommand{\Ea}[2]{\ensuremath{\mathbb{E}_{#1}\!\left[#2\right]}}% expectation operator
\newcommand{\F}[1]{\ensuremath{\mathcal{F}\!\left\{#1\right\}}}% Fourier transform operator
\newcommand{\IF}[1]{\ensuremath{\mathcal{F}^{-1}\!\left\{#1\right\}}}% inverse Fourier transform operator
\newcommand{\var}[1]{\ensuremath{\text{var}\!\left\{#1\right\}}}% variance operator
\newcommand{\cov}[1]{\ensuremath{\text{cov}\!\left\{#1\right\}}}% covariance operator
\newcommand{\corr}[1]{\ensuremath{\text{corr}\!\left\{#1\right\}}}% correlation operator
\newcommand{\avg}[1]{\ensuremath{\text{avg}\!\left\{#1\right\}}}% averaging operator
\newcommand{\avgvar}[1]{\ensuremath{\overline{\text{var}}\!\left\{#1\right\}}}% average variance operator
\renewcommand{\Re}[1]{\ensuremath{\text{Re}\!\left[#1\right]}}% real part
\renewcommand{\Im}[1]{\ensuremath{\text{Im}\!\left[#1\right]}}% imaginary part

\newcommand{\Rk}[1]{\ensuremath{\text{rank}\{#1\}}}%rank operator
\newcommand{\RkLR}[1]{\ensuremath{\text{rank}\bigl\{#1\bigr\}}}%rank operator
\newcommand{\Tr}[1]{\ensuremath{\text{tr}\bigl[#1\bigr]}}%trace operator
\newcommand{\norm}[2]{\ensuremath{\lVert #1 \rVert^{#2}}}%norm operator
\newcommand{\inprod}[2]{\ensuremath{\bigl\langle #1 \bigr\rangle_{#2}}}%inner product
\newcommand{\abs}[1]{\ensuremath{\lvert#1\rvert}} %absolute value
% numbers and states
\newcommand{\REAL}{\ensuremath{\mathbb{R}}}% real numbers
\newcommand{\NATURAL}{\ensuremath{\mathbb{N}}}% natural numbers
\newcommand{\INTEGER}{\ensuremath{\mathbb{Z}}}% integer numbers (natural numbers plus zero)
\newcommand{\COMPLEX}{\ensuremath{\mathbb{C}}}% complex numbers
\newcommand{\IMAG}{\ensuremath{\mathbb{I}}}% imaginary numbers

\newcommand{\calli}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\HS}[1]{\ensuremath{\mathcal{H}_{#1}}} %hypothesis 
\newcommand{\HILB}{\ensuremath{\mathcal{H}}} %Hilbert space

\newcommand{\GAUSS}[2]{\ensuremath{\mathcal{N}\left(#1,#2\right)}} %normal distribution

\newcommand{\Real}{\mathcal{R}}
\newcommand{\Imag}{\mathcal{I}}

% other
\newcommand{\conj}{\ensuremath{^\ast}}% conjugate complex
\newcommand{\transp}{\ensuremath{^\mathsf{T}}}% normal vector transpose
\newcommand{\conjt}{\ensuremath{^\mathsf{H}}}% conjugate (Hermitian) transpose
\newcommand{\mtx}[2]{\left[\ensuremath{\begin{array}{#1}#2\end{array}}\right]}%vector/matrix
\newcommand{\mtxt}[1]{\ensuremath{\bigl[\,#1\,\bigr]}}%vector/matrix for inline definition
\newcommand{\isdef}{\ensuremath{\mathrel{:=}}}% definition left->right
\newcommand{\isdefflip}{\ensuremath{\mathrel{=:}}}% definition right->left
\newcommand{\isreq}{\ensuremath{\mathrel{\stackrel{!}{=}}}}% is required
\newcommand{\textrel}[1]{\ensuremath{{\;{#1}\;}}}% relation symbol for in-line equations (fixed spacing)

\newcommand{\topmidbot}[3]{\underset{#3}{\overset{#1}{#2}}} %stacking three
\newcommand{\limit}[1]{\ensuremath{\underset{#1}{\text{lim}}}} %limes

% statistics
\newcommand{\pdf}[1]{\ensuremath{p\!\left(#1\right)}}
\newcommand{\PR}[1]{\ensuremath{P\!\left(#1\right)}}



% variables
\newcommand{\FIM}{J}
\newcommand{\EFIM}{J}

% definitions for FIM results
\newcommand{\Aaa}{\FIM_{\phi \phi,m}}
\newcommand{\Aab}{\FIM_{\phi \tau,m}}
\newcommand{\Aba}{\FIM_{\tau \phi,m}}
\newcommand{\Abb}{\FIM_{\tau \tau,m}}
\newcommand{\Am}{\mtx{cc}{\Aaa & \Aab \\ \Aba & \Abb}}
\newcommand{\AmO}{\mtx{cc}{\FIM_{\phi \phi} & 0 \\ 0 & \FIM_{\tau \tau}}}

\newcommand{\Baa}{\FIM_{\phi \psi,m}}
\newcommand{\Bab}{\FIM_{\phi \Real \alpha,m}}
\newcommand{\Bac}{\FIM_{\phi \Imag \alpha,m}}
\newcommand{\Bbbnew}{\FIM_{\tau \Real \alpha,m}} % \Bbb seems to be defined in package bm...
\newcommand{\Bbc}{\FIM_{\tau \Imag \alpha ,m}}
\newcommand{\balpha}{\vm{b}_{\alpha}}
% \newcommand{\Bba}{I_{\phi \psi,m}}
% \newcommand{\Bm}{\mtx{ccc}{\Baa & \Bab & \Bac \\ \Bba & \Bbbnew & \Bbc}}
\newcommand{\Bm}{\mtx{cc}{\Bab & \Bac \\ \Bbbnew & \Bbc}}
\newcommand{\BmO}{\mtx{cc}{0 & 0 \\ \FIM_{\tau \Real \alpha} & \FIM_{\tau \Imag \alpha}}}

\newcommand{\Caa}{\FIM_{\psi \psi,m}}
\newcommand{\Cab}{0}
\newcommand{\Cac}{0}
\newcommand{\Cba}{0}
\newcommand{\Cbb}{\FIM_{\Real \alpha \Real \alpha,m}}
\newcommand{\Cbc}{\FIM_{\Real \alpha \Imag \alpha,m}}
\newcommand{\Cca}{0}
\newcommand{\Ccb}{\FIM_{\Imag \alpha \Real \alpha,m}}
\newcommand{\Ccc}{\FIM_{\Imag \alpha \Imag \alpha,m}}
% \newcommand{\Cm}{\mtx{ccc}{\Caa & \Cab & \Cac \\ \Cba & \Cbb & \Cbc \\ \Cca & \Ccb & \Ccc}}
\newcommand{\Cm}{\mtx{cc}{\Cbb & \Cbc \\ \Ccb & \Ccc}}
\newcommand{\CmO}{\mtx{cc}{\FIM_{\Real \alpha \Real \alpha} & 0 \\ 0 & \FIM_{\Imag \alpha \Imag \alpha}}}

% \newcommand{\fim}{\ensuremath{\vms{\mathcal{I}}}}
\newcommand{\fim}{\ensuremath{\vm{J}}}
\newcommand{\efim}{\ensuremath{\vm{J}}}

\newcommand{\DT}{\Delta T}

\newcommand{\minus}{\rmv - \rmv}

\newcommand{\s}{\hspace*{0.5pt}}

\newcommand{\pe}{p_{\text{E}}(u_n^{(j)}\rmv\rmv\rmv,q_n^{(j)})}
\newcommand{\perv}{p_{\text{E}}(\rv{u}_n^{(j)}\rmv\rmv\rmv, \rv{q}_n^{(j)})}
\newcommand{\pd}{p_{\text{D}}({u}_{k,n}^{(j)})}
\newcommand{\pdrv}{p_{\text{D}}(\rv{u}_{k,n}^{(j)})}
\newcommand{\sigmadhat}{\hat{\sigma}_{\text{d}\s n,m}^{(j)}}
\newcommand{\dlos}{d^{(j)}_{\text{LOS}\s n}(\bm{p}_n)}
\newcommand{\sigmaahat}{\hat{\sigma}_{\mathrm{\alpha}\s n,m}^{(j)}}
\newcommand{\dr}{\gamma_r}
\newcommand{\df}{\gamma_f}

\providecommand{\norm}[1]{\lVert#1\rVert}
\newtheorem{problem}{\noindent \textbf{Problem}}
\newtheorem{theorem}{\noindent \textbf{Theorem}}
%\newtheorem{algorithm1}{\noindent \textbf{Algorithm}}
\newtheorem{lemma}{\noindent \textbf{Lemma}}
\newtheorem{conjecture}{\noindent \textbf{Conjecture}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\estpdf}[1]{f_{\hat{\mathsf{d}}|\bm{\mathsf{x}}}(#1|\bm{x})}
\newcommand{\likepdf}[1]{f_{\bm{\mathsf{x}}}(#1)}

\newcommand{\disppar}{\psi}
\newcommand{\zd}{\ensuremath{{z_\tau^{(j)}}_{\rmv\rmv\rmv\rmv\rmv\rmv\rmv  m,n}}}
\newcommand{\zu}{\ensuremath{{z_\mathrm{u}^{(j)}}_{\rmv\rmv\rmv\rmv\rmv\rmv\rmv m,n}}}
\newcommand{\zdr}{\ensuremath{{\rv{z}_\tau^{(j)}}_{\rmv\rmv\rmv\rmv\rmv\rmv\rmv  m,n}}}
\newcommand{\zur}{\ensuremath{{\rv{z}_\mathrm{u}^{(j)}}_{\rmv\rmv\rmv\rmv\rmv\rmv\rmv m,n}}}
\newcommand{\zdOne}{\ensuremath{{z_\tau^{(1)}}_{\rmv\rmv\rmv\rmv\rmv\rmv\rmv  m,n}}}
\newcommand{\zdOneTwoHundred}{\ensuremath{{z_\tau^{(1)}}_{\rmv\rmv\rmv\rmv\rmv\rmv\rmv  200,m}}}
\newcommand{\zuZero}{\ensuremath{{z_\mathrm{u}^{(j)}}_{\rmv\rmv\rmv\rmv\rmv\rmv\rmv 0,m}}}
\newcommand{\zdZero}{\ensuremath{{z_\tau^{(j)}}_{\rmv\rmv\rmv\rmv\rmv\rmv\rmv  0,m}}}
\newcommand{\zuZeroMax}{\ensuremath{{{z}_\mathrm{u}^{(j)}}_{\rmv\rmv\rmv\rmv\rmv\rmv\rmv 0, \text{max}}}}
 

\newcommand{\scale}{0.6}
\newcommand{\bkm}{\scalebox{\scale}{$b^{(j)}_{l,n} = \underline{K} + m$}}
\newcommand{\scb}{\scalebox{\scale}{$b^{(j)}_{l,n}$}}
\newcommand{\bi}{\scalebox{\scale}{$b^{(j)}_{l,n} = i$}}

\newcommand{\sdnrp}{\ensuremath{\omega}}
\newcommand{\sdnr}[1]{\ensuremath{\omega_n^{(j)\s #1}}}
\newcommand{\sdnrr}[1]{\ensuremath{\rv{\omega}_n^{(j)\s #1}}}
\newcommand{\sdnrt}[1]{\ensuremath{\tilde{\omega}_n^{(j\s #1)}}}

\newcommand{\noise}{\ensuremath{n}}


==> inputFiles/Wgroup-Teaching-Preamble.tex <==
% Greek lowercase letters, sans serif font - by Guido

%\@ifpackageloaded{<name>}{<true>}{<false>}
\usepackage{bm}

%% =========== Euler ==========
%\DeclareMathAlphabet{\matheur}{U}{eur}{m}{n}
%\SetMathAlphabet{\matheur}{bold}{U}{eur}{b}{n}
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\matheur{#1}\fi%for math sans serif (Euler)
%}
%% =========================
%
%% ==== Computer Modern Sans Serif ====
\DeclareMathAlphabet{\mathsfbr}{OT1}{cmss}{m}{n}%for math sans serif (cmss)
\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmss}{bx}{n}%for math sans serif (cmss)
\DeclareRobustCommand{\msf}[1]{%
  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif (cmss)
}
%% =========================

% ==== Computer Modern Bright ====
%% Part 1: This is necessary to fix a bug in the .fd file of the font!!!
%\DeclareFontFamily{OT1}{cmbr}{\hyphenchar\font45 }
%\DeclareFontShape{OT1}{cmbr}{m}{n}{%
%  <-9>cmbr8
%  <9-10>cmbr9
%  <10-17>cmbr10
%  <17->cmbr17
%}{}
%\DeclareFontShape{OT1}{cmbr}{m}{sl}{%
%  <-9>cmbrsl8
%  <9-10>cmbrsl9
%  <10-17>cmbrsl10
%  <17->cmbrsl17
%}{}
%\DeclareFontShape{OT1}{cmbr}{m}{it}{%
%  <->ssub*cmbr/m/sl
%}{}
%\DeclareFontShape{OT1}{cmbr}{b}{n}{%
%  <->ssub*cmbr/bx/n
%}{}
%\DeclareFontShape{OT1}{cmbr}{bx}{n}{%
%  <->cmbrbx10
%}{}
%% Part 2
%\DeclareMathAlphabet{\mathsfbr}{OT1}{cmbr}{m}{n}%for math sans serif bright (cmbr)
%\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmbr}{b}{n}%for math sans serif bright (cmbr)
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif bright (cmbr)
%}
%% =========================

\makeatletter
\newcommand{\msfgreek}[1]{\csname s\expandafter\@gobble\string#1\endcsname}
\makeatother

% Sans serif greek
\DeclareFontEncoding{LGR}{}{} % or load \usepackage{textgreek}
\DeclareSymbolFont{sfgreek}{LGR}{cmss}{m}{n}
\SetSymbolFont{sfgreek}{bold}{LGR}{cmss}{bx}{n}
\DeclareMathSymbol{\salpha}{\mathord}{sfgreek}{`a}
\DeclareMathSymbol{\sbeta}{\mathord}{sfgreek}{`b}
\DeclareMathSymbol{\sgamma}{\mathord}{sfgreek}{`g}
\DeclareMathSymbol{\sdelta}{\mathord}{sfgreek}{`d}
\DeclareMathSymbol{\sepsilon}{\mathord}{sfgreek}{`e}
\DeclareMathSymbol{\szeta}{\mathord}{sfgreek}{`z}
\DeclareMathSymbol{\seta}{\mathord}{sfgreek}{`h}
\DeclareMathSymbol{\stheta}{\mathord}{sfgreek}{`j}
\DeclareMathSymbol{\siota}{\mathord}{sfgreek}{`i}
\DeclareMathSymbol{\skappa}{\mathord}{sfgreek}{`k}
\DeclareMathSymbol{\slambda}{\mathord}{sfgreek}{`l}
\DeclareMathSymbol{\smu}{\mathord}{sfgreek}{`m}
\DeclareMathSymbol{\snu}{\mathord}{sfgreek}{`n}
\DeclareMathSymbol{\sxi}{\mathord}{sfgreek}{`x}
\DeclareMathSymbol{\somicron}{\mathord}{sfgreek}{`o}
\DeclareMathSymbol{\spi}{\mathord}{sfgreek}{`p}
\DeclareMathSymbol{\srho}{\mathord}{sfgreek}{`r}
\DeclareMathSymbol{\ssigma}{\mathord}{sfgreek}{`s}
\DeclareMathSymbol{\stau}{\mathord}{sfgreek}{`t}
\DeclareMathSymbol{\supsilon}{\mathord}{sfgreek}{`u}
\DeclareMathSymbol{\sphi}{\mathord}{sfgreek}{`f}
\DeclareMathSymbol{\schi}{\mathord}{sfgreek}{`q}
\DeclareMathSymbol{\spsi}{\mathord}{sfgreek}{`y}
\DeclareMathSymbol{\somega}{\mathord}{sfgreek}{`w}
\let\svarepsilon\sepsilon
\let\svartheta\stheta
\let\svarpi\spi
\let\svarrho\srho
\DeclareMathSymbol{\svarsigma}{\mathord}{sfgreek}{`c}
\let\svarphi\sphi
\DeclareMathSymbol{\sGamma}{\mathalpha}{sfgreek}{`G}
\DeclareMathSymbol{\sDelta}{\mathalpha}{sfgreek}{`D}
\DeclareMathSymbol{\sTheta}{\mathalpha}{sfgreek}{`J}
\DeclareMathSymbol{\sLambda}{\mathalpha}{sfgreek}{`L}
\DeclareMathSymbol{\sXi}{\mathalpha}{sfgreek}{`X}
\DeclareMathSymbol{\sPi}{\mathalpha}{sfgreek}{`P}
\DeclareMathSymbol{\sSigma}{\mathalpha}{sfgreek}{`S}
\DeclareMathSymbol{\sUpsilon}{\mathalpha}{sfgreek}{`U}
\DeclareMathSymbol{\sPhi}{\mathalpha}{sfgreek}{`F}
\DeclareMathSymbol{\sPsi}{\mathalpha}{sfgreek}{`Y}
\DeclareMathSymbol{\sOmega}{\mathalpha}{sfgreek}{`W}

\DeclareRobustCommand{\mcal}[1]{%
  \ifcat\noexpand#1\relax\mathnormal{#1}\else\cal{#1}\fi
}
\DeclareRobustCommand{\BM}[1]{%
  \ifcat\noexpand#1\relax\bm{\boldUppercaseItalicGreek{#1}}\else\bm{#1}\fi
}
\makeatletter
\newcommand{\boldUppercaseItalicGreek}[1]{\csname var\expandafter\@gobble\string#1\endcsname}
\makeatother
%-------------------------
% Math symbol
%-------------------------
%\newcommand{\rv}[1]{\MakeLowercase{\msf{#1}}}  
%\newcommand{\RV}[1]{\bm{\MakeLowercase{\msf{#1}}}}
%\newcommand{\RM}[1]{\bm{\MakeUppercase{\msf{#1}}}}
%\newcommand{\RS}[1]{\MakeUppercase{\msf{#1}}}
\newcommand{\rv}[1]{\msf{#1}}
\newcommand{\RV}[1]{\bm{\msf{#1}}}
\newcommand{\RM}[1]{\bm{\msf{#1}}}
\newcommand{\RS}[1]{\msf{#1}}

\newcommand{\V}[1]{\bm{#1}}
\newcommand{\M}[1]{\BM{#1}}
\newcommand{\Set}[1]{{\mcal{#1}}}


==> inputFiles/geom_model.tex <==
%!TEX root = ../JAIF_2023_V3.tex

\section{Geometrical Relations}\label{sec:geometricRel} 

At each time $n$, we consider a mobile agent at position $\V{p}_n$ equipped with an \bl{antenna array} and $J$ base stations, called \acp{pa}, equipped with an \bl{antenna array} and at known positions $\V{p}_{\mathrm{pa}}^{(j)} = \big[ {p}_{1,\mathrm{pa}}^{(j)} \ist\ist\ist {p}_{2,\mathrm{pa}}^{(j)} \big]^{\mathrm{T}} \rmv\rmv\in \mathbb{R}^2\rmv$, $j \rmv\in\rmv \{1,\ldots,J\}$, where $J$ is assumed to be known, in an environment described by reflective surfaces. 
Specular reflections of radio signals at flat surfaces are modeled by \acp{va} that are mirror images of \acp{pa}. 
In particular, \ac{va} positions associated to single-bounce reflections are given by
\vspace*{-1mm}
\begin{align}
	\V{p}^{(j)}_{l,\mathrm{va}} &= \V{p}^{(j)}_{\mathrm{pa}} + 2\big( \V{u}_l^{\T}\V{e}_l - \V{u}_l^{\T}\V{p}^{(j)}_{\mathrm{pa}}\big)\V{u}_l \label{eq:VA1BPAequation}
	\\[-7mm]
	\nn
\end{align}
where $\V{u}_l$ is the normal vector of the according reflective surface, and $\V{e}_l$ is an arbitrary point on this surface. 
The second summand in \eqref{eq:VA1BPAequation} represents the normal vector w.r.t. this reflective surface in direction $\V{u}_l$ with the length of two times the distance between \ac{pa} $j$ at position $\V{p}^{(j)}_{\mathrm{pa}}$ and the normal-point at the reflective surface, i.e., $2\big( \V{u}_l^{\T}\V{e}_l - \V{u}_l^{\T}\V{p}^{(j)}_{\mathrm{pa}}\big)$. 
An example is shown in Fig.~\ref{fig:fp}. \ac{va} positions associated to multiple-bounce reflections are determined by applying \eqref{eq:VA1BPAequation} multiple times. The current number of \textit{visible} \acp{va}\footnote{A \ac{va} does not exist at time $n$, when the reflective surface corresponding to this \ac{va} is obstructed with respect to the agent.} within the scenario (associated with single-bounce and higher-order bounce reflections) is $L_n^{(j)}$ for each of the $J$ \acp{pa}.




\begin{figure}[t]
	\centering   
	\ifthenelse{\equal{\arxiv}{false}}
		{  
	\subfloat[]{
		\tikzsetnextfilename{indoor_environment_MPAs}
		\scalebox{1}{\input{./plots/indoor_environment_MPAs.tex}}
		\label{fig:fp}}%\hfill
	\vspace*{2mm}	
	\subfloat[]{\centering
		\tikzsetnextfilename{environment_signal_example_seed3_log}
		\setlength{\figurewidth}{0.8\columnwidth}
		\setlength{\figureheight}{0.22\columnwidth}%0.275  
		\def\datapath{./plots/signal_examples/environment_signal_example_seed3_log}
		\hspace{-18mm}{\input{\datapath/environment_signal_example_seed3_log.tex}}\vspace{-1mm}
		\label{fig:signal}}	}
		{ 	\subfloat[]{
		\scalebox{1}{\includegraphics{./compiledPlots/indoor_environment_MPAs.pdf}}
		\label{fig:fp}}%\hfill
	\vspace*{2mm}	
	\subfloat[]{\centering
		\setlength{\figurewidth}{0.8\columnwidth}
		\setlength{\figureheight}{0.22\columnwidth}%0.275  
		\hspace{-18mm}{\includegraphics{./compiledPlots/environment_signal_example_seed3_log.pdf}}\vspace{-1mm}
		\label{fig:signal}}	}
	\vspace*{-1.5mm}
	\caption{Exemplary indoor environment \sref{fig:fp} and representative realization of a received signal \sref{fig:signal}. The floor plan\vspace*{0.3mm} in \sref{fig:fp} includes an agent at position $\V{p}_n$ and a \ac{pa} at position \smash{$\V{p}^{(j)}_\text{pa}$} and two \acp{va} at positions \smash{$\V{p}^{(j)}_{l,\text{va}}$} for corresponding surfaces. The signal shown in \sref{fig:signal}\vspace*{0.3mm} is received by \ac{pa} at position \smash{$\V{p}^{(j)}_\text{pa}$}. Non-ideal antennas or reflective surfaces as indicated in \sref{fig:fp} by generic impulse responses $h_{\text{ant}, n}^{(j)}(\tau)$ and $h_{\text{surf}, n}^{(j)}(\tau)$ lead to the received signal {$\RV{s}_{\text{rx},n}^{(j)}$} shown in \sref{fig:signal} (c.f. received signal without dispersion). Resulting measurements (\ac{mpc} parameter estimates)\vspace*{0.3mm} $\V{z}^{(j)}_{m,n}$ are indicated in the received signal {$\RV{s}_{\text{rx},n}^{(j)}$} shown in \vspace*{0.3mm} \sref{fig:signal} alongside the proposed dispersion model.}
	\vspace*{-4mm}
	\label{fig:overview}
\end{figure}


